Class Attention to Regions of Lesion for Imbalanced Medical Image Recognition

Automated medical image classification is the key component in intelligent diagnosis systems. However, most medical image datasets contain plenty of samples of common diseases and just a handful of rare ones, leading to major class imbalances. Currently, it is an open problem in intelligent diagnosis to effectively learn from imbalanced training data. In this paper, we propose a simple yet effective framework, named \textbf{C}lass \textbf{A}ttention to \textbf{RE}gions of the lesion (CARE), to handle data imbalance issues by embedding attention into the training process of \textbf{C}onvolutional \textbf{N}eural \textbf{N}etworks (CNNs). The proposed attention module helps CNNs attend to lesion regions of rare diseases, therefore helping CNNs to learn their characteristics more effectively. In addition, this attention module works only during the training phase and does not change the architecture of the original network, so it can be directly combined with any existing CNN architecture. The CARE framework needs bounding boxes to represent the lesion regions of rare diseases. To alleviate the need for manual annotation, we further developed variants of CARE by leveraging the traditional saliency methods or a pretrained segmentation model for bounding box generation. Results show that the CARE variants with automated bounding box generation are comparable to the original CARE framework with \textit{manual} bounding box annotations. A series of experiments on an imbalanced skin image dataset and a pneumonia dataset indicates that our method can effectively help the network focus on the lesion regions of rare diseases and remarkably improves the classification performance of rare diseases.

==> figures/arch.tex <==
\begin{figure*}[ht]
	\centering
	\includegraphics[width=1.0\linewidth]{img/vgg19_arch.pdf}
	\caption{Architecture of the ResNet50 backbone.}
	\label{fig:arch}
\end{figure*}


==> figures/datasets.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\textwidth]{./img/dataset.pdf}
    \caption{The imbalanced data distribution of two commonly used medical image datasets: (a) Skin dataset, and (b) Pneumonia Chest X-ray dataset. NV: Melanocytic nevus; MEL: Melanoma; BKL: Benign keratosis (solar lentigo/seborrheic keratosis/lichen planus-like keratosis); BCC: Basal cell carcinoma; AKIEC: Actinic keratosis/Bowen’s disease (intraepithelial carcinoma);  VASC: Vascular lesion; DF: Dermatofibroma.}
    \label{fig:dataset}
\end{figure}


==> figures/details.tex <==
\begin{figure}[h]
	\centering
	\includegraphics[scale=0.9]{./img/details.pdf}
	\caption{For the Skin Dataset, Mean Class Accuracy over the whole dataset and Recall for each class by cost sensitive learning(CLS), and CARE based on cost sensitive learning(CLS)}
	\label{tab:r26}
\end{figure}

==> sec/acknowledgement.tex <==
\section*{Acknowledgment}
This work is supported in part by the National Key Research and Development Program (grant No. 2018YFC1315402), the Guangdong Key Research and Development Program (grant No. 2019B020228001), the National Natural Science Foundation of China (grant No. U1811461), and the Guangzhou Science and Technology Program (grant No. 201904010260)

==> tables/decouple.tex <==
	\begin{table*}[h]
		\centering
		\caption{Comparison with a well known data imbalance strategy on the Skin Dataset.}
		\label{tab:decouple}
		\small
		\begin{tabular}{ccccccccc}
			\toprule
			\multirow{2}{*}{$\lambda$} & \multirow{2}{*}{\textbf{MCA}} & \multicolumn{7}{c}{ \textbf{Recall} } \\
		\cline { 3 - 9 }  & & DF & VASC & AKIE & BCC & PBK & MEL & NV \\		
			\midrule
			\rowcolor{mygray} Baseline & 72.7 & 52.1 & 86.2 & 53.0 & 85.4 & 70.0 & 61.8 & 97.5\\
			Decouple & 73.9 & 65.2 & 82.7 & 57.5 & 81.5 & 76.3 & 63.2 & 91.9\\
			CARE(Ours) & \textcolor{red}{78.3} & \textcolor{red}{73.9} & 89.6 & 62.1 & 83.4 & 74.0 & 73.0 & 92.2\\
			\bottomrule
		\end{tabular}
	\end{table*}  

==> tables/detail_f.tex <==
\begin{table}[h]
		\centering
		\caption{Training details of the second stage on the Skin dataset}
		\label{tab:r292}
        \scriptsize
		\begin{tabular}{l|l}
		config & value\\
		\hline
		optimizer & AdamW\\
		base learning rate & 1e-4\\
%		weight decay & \\
		optimizer momentum & (0.9, 0.999)\\
		batch size & 96\\
		training epochs & 200 \\
%		augmentation & \texttt{Resize(224, 224)}\\
		attention feature map & 224$\times$ 224\\
		$\alpha$ & 0.5\\
		$\lambda$ & 1\\
		$\tau$ & 0.7\\
		\end{tabular}
\end{table}

==> tables/details_p.tex <==
\begin{table}[h]
		\centering
		\caption{Training details of the first stage}
		\label{tab:r29}
        % \small
        \scriptsize
		\begin{tabular}{l|l}
		config & value\\
		\hline
		optimizer & AdamW\\
		base learning rate & 1e-4\\
%		weight decay & \\
		optimizer momentum & (0.9, 0.999)\\
		batch size & 96\\
		training epochs & 200 \\
		\end{tabular}
	
\end{table}


